CFD analysis of electroviscous effects in pressure-driven flow of electrolyte liquid through an asymmetrically charged non-uniform microfluidic device

The electroviscous effects in the pressure-driven flow of electrolyte liquid through an asymmetrically charged contraction-expansion (4:1:4) slit microfluidic device have been investigated numerically. The mathematical model (i.e., Poisson's, Navier-Stokes, and Nernst-Planck equations) is solved using the finite element method to obtain the electrical potential, velocity, pressure, ion concentration fields, excess charge, an induced electric field strength for the following ranges of parameters: Reynolds number (${Re=0.01}$), Schmidt number (${\mathit{Sc}=1000}$), inverse Debye length (${2\le K\le 20}$), top wall surface charge density (${4\le S_t\le 16}$), surface charge ratio (${0\le S_r\le 2}$) and contraction ratio (${d_{\text{c}}=0.25}$). Results show that the charge asymmetry at the different walls of the microfluidic device plays a significant role in the induced electric field development and microfluidic hydrodynamics. The total potential (${|\Delta U|}$) and pressure drop (${|\Delta P|}$) maximally increase by 197.45\% and 25.46\%, respectively, with asymmetry of the charge. {The electroviscous correction factor (ratio of apparent to physical viscosity) maximally increases by 20.85\% (at ${K=2}$, ${S_t=16}$ for ${0\le S_r\le 2}$), 25.46\% (at ${S_t=16}$, ${S_r=2}$ for ${2\le K\le 20}$), and 39.13\% (at ${K=2}$, ${S_r=2}$ for ${0\le S_t\le16}$).} Further, a simpler analytical model is developed to predict the pressure drop in electroviscous flow considering asymmetrically charged surface, based on the Poiseuille flow in the individual uniform sections and pressure losses due to orifice, estimates the pressure drop 1--2\% within the numerical results. The robustness of this model enables the use of present numerical results for design aspects in microfluidic applications.

==> Makefile <==
# type "make" command in Unix to create ps and pdf file 
#
#Colors
gray=\e[1;30m
red=\e[0;31m
RED=\e[1;31m
blue=\e[0;34m
BLUE=\e[1;34m
green=\e[0;32m
GREEN=\e[1;32m
cyan=\e[0;36m
CYAN=\e[1;36m
NC=\e[0m # No Color

# the documents to be compiled by default
# set defaultfile to the name of the main file without the .tex
#
defaultfile = $(foreach i,$(filter-out ,$(shell grep -l documentclass *.tex)), $(basename $i))
#
ASPELL = aspell -t -c --mode=tex
ISPELL = ispell -t  --mode=tex
LATEX = latex -interaction=batchmode
BIBTEX = bibtex 
MAKEINDEX = makeindex
PDFLATEX = pdflatex -interaction=batchmode
#
DVIPS = dvips -Pwww
DVIPDF = dvipdf 
PSPDF = ps2pdf
#
all: pdf clean
#
pdf:
	@echo -e ""
	@echo -e "$(BLUE)====> Default file being compiled: $(RED)$(defaultfile).tex$(NC)"
	@echo -e ""
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running BibTex$(NC)" ;
	$(BIBTEX) $< $(QUIET)$(defaultfile)
#	
#	@echo -e "$(BLUE)====> $(green)Running aspell$(NC)" ;
#	$(ASPELL) $< $(QUIET)$(defaultfile).tex
#
#	@echo -e "$(BLUE)====> $(green)Running ispell$(NC)" ;
#	$(ISPELL) $< $(QUIET)$(defaultfile).tex
#
	@echo -e "$(BLUE)====> $(green)Running Makeindex$(NC)" ;
	$(MAKEINDEX) $< $(QUIET)$(defaultfile).nlo -s nomencl.ist -o  $(QUIET)$(defaultfile).nls
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PS document from DVI document$(NC)" ;
	$(DVIPS) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PDF document from DVI document$(NC)" ;
	$(DVIPDF) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Generating PDF document from PS document$(NC)" ;
#	$(PSPDF) $(defaultfile).ps $(defaultfile).pdf
#
clean:
	@echo -e "$(RED)====> $(red)Cleaning up temporary files$(NC)"
	rm -f *.brf *.glo *.ist *.nlo  *.out *.spl *.log *.aux *.*% *.lof *.gls *.nls
	rm -f *.lop *.lot *.toc *.idx *.ilg *.ind *.bbl *.blg *.backup *.bak *~



